Attention Filtering for Multi-person Spatiotemporal Action Detection on Deep Two-Stream CNN Architectures

Action detection and recognition tasks have been the target of much focus in the computer vision community due to their many applications, namely, security, robotics and recommendation systems. Recently, datasets like AVA, provide multi-person, multi-label, spatiotemporal action detection and recognition challenges. Being unable to discern which portions of the input to use for classification is a limitation of two-stream CNN approaches, once the vision task involves several people with several labels. We address this limitation and improve the state-of-the-art performance of two-stream CNNs. In this paper we present four contributions: our fovea attention filtering that highlights targets for classification without discarding background; a generalized binary loss function designed for the AVA dataset; miniAVA, a partition of AVA that maintains temporal continuity and class distribution with only one tenth of the dataset size; and ablation studies on alternative attention filters. Our method, using fovea attention filtering and our generalized binary loss, achieves a relative video mAP improvement of 20% over the two-stream baseline in AVA, and is competitive with the state-of-the-art in the UCF101-24. We also show a relative video mAP improvement of 12.6% when using our generalized binary loss over the standard sum-of-sigmoids.

==> Acronyms.tex <==
% #############################################################################
% This is the ACRONYMS Definition
% !TEX root = ../main.tex
% #############################################################################

\begin{multicols}{2}
\begin{acronym}[ILSVRC]
    \acro{BB}{Bounding Box}
    \acro{COCO}{Common Objects In Context}
	\acro{CNN}{Convolutional Neural Network}
    \acro{ILSVRC}{Imagenet's Large Scale Visual Recognition Challenge}
	\acro{IoU}{Intersection over Union}
	\acro{mAP}{mean Average Precision}
	\acro{MDP}{Markov decision process}
	\acro{RoI}{Region of Interest}
	\acro{RPN}{Region Proposal Network}
	\acro{SSD}{Single Shot Detector}
	\acro{OF}{Optical Flow}
    \acro{FC}{Fully-Connected}
    \acro{NHU}{Number of Hidden Units}
    \acro{MLP}{Multi-Layer Perceptron}
    \acro{RNN}{RNN}{Recurrent Neural Network}
    \acro{LSTM}{LSTM}{Long-short term memory}
    \acro{TSN}{TSN}{Temporal Segment Network}
    \acro{R-CNN}{R-CNN}{Region-Convolutional Neural Network}
    \acro{MLD}{Multi-label dataset}
    \acro{SLD}{Single-label dataset}
    \acro{BPTT}{Backpropagation Through Time}
    \acro{SVM}{Support Vector Machines}
    \acro{RF}{Random Forests}
    \acro{AVA}{Atomic Visual Actions}
    \acro{GPU}{Graphics Processing Unit}
    \acro{UCF}{University of Central Florida}
    \acro{BB}{Bounding Box}
    \acro{AP}{Average Precision}
    \acro{iDT}{improved Dense Trajectories}
    \acro{FPS}{Frames Per Second}
    \acro{GBB}{Gaussian Background Blur}
\end{acronym}
\end{multicols}


